Multi-Message Shuffled Privacy in Federated Learning

We study differentially private distributed optimization under communication constraints. A server using SGD for optimization aggregates the client-side local gradients for model updates using distributed mean estimation (DME). We develop a communication-efficient private DME, using the recently developed multi-message shuffled (MMS) privacy framework. We analyze our proposed DME scheme to show that it achieves the order-optimal privacy-communication-performance tradeoff resolving an open question in [1], whether the shuffled models can improve the tradeoff obtained in Secure Aggregation. This also resolves an open question on the optimal trade-off for private vector sum in the MMS model. We achieve it through a novel privacy mechanism that non-uniformly allocates privacy at different resolutions of the local gradient vectors. These results are directly applied to give guarantees on private distributed learning algorithms using this for private gradient aggregation iteratively. We also numerically evaluate the private DME algorithms.

==> Binary_vectors.tex <==
\section{Binary vectors}~\label{sec:binary_vector}
In this section, we assume that each client has a binary vector $\mathbf{b}_i\in\lbrace 0,1\rbrace^{d}$. The server wants to estimate the mean $\overline{\mathbf{b}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{b}_i$ under privacy and communication constraints. This problem is a generalization to the scalar binary summation problem~\cite{cheu2019distributed}. The straightforward solution is to apply the scalar solution for each coordinate separately. However, this solution requires $d$ bits per client. Our goal in this section is to design private mechanisms with different communication budget per client.

The client-side mechanism is presented in Algorithm~\ref{algo:binary_vector}, where the parameter $s$ determines the communication budget for each client and the parameter $p$ determines the total privacy budget (see Theorem~\ref{thm:binary_vector_ldp}). For given $s\in\lbrace 1,\ldots,d\rbrace$, each client splits the binary vector $\mathbf{b}_i$ into $s$ sub-vectors each with dimension $a = \lceil \frac{d}{s}\rceil$. Then, the client chooses uniformly at random one coordinate from each sub-vector and privatizes its bit using the 2RR mechanism~\ref{sec:binary_rr}. Observe that the output of Algorithm~\ref{algo:binary_vector} can be represented as a sparse $d$-dimensional vector with only $s$ non-zero bits.

When $s=1$, then each client applies the 2RR mechanism on each coordinate separately. On the other hand, when $s=d$, the client chooses uniformly at random one coordinate and applies the 2RR mechanism. Thus, we get trade-offs between privacy-communication and accuracy. The server aggregator $\mathcal{A}^{\text{Bin}}$ is presented in Algorithm~\ref{algo:binary_vector_sum_server}, where the server simply aggregates the received randomized bits. 

\begin{algorithm}[t]
\caption{: Local Randomizer $\mathcal{R}^{\text{Bin}}_{p,s}$ }\label{algo:binary_vector}
\begin{algorithmic}[1]
\STATE \textbf{Public parameter:} Privacy parameter $p$, and communication budget $s$.
\STATE \textbf{Input:} $\mathbf{b}_i\in\lbrace 0,1\rbrace^{d}$.
\STATE $a\gets \lceil \frac{d}{s}\rceil$
\STATE If $a$ is not integer, add $(sa-d)$ dummy zeros to the binary vector $\mathbf{b}$.
\FOR{$j\in [s]$}
\STATE Choose uniformly at random one coordinate $z_{ij}\gets\mathsf{Unif}\left(\lbrace (j-1)a,\ldots,ja\rbrace\right)$.
\STATE $y_{ij}\gets a\mathcal{R}^{\textsl{2RR}}_p\left(\mathbf{b}_i[z_{ij}]\right)$
\ENDFOR
\STATE \textbf{Return:} The client sends $s$ messages $\mathcal{Y}_i\gets\left\{\left(z_{i1},y_{i1}\right),\ldots,\left(z_{is},y_{is}\right)\right\}$.
\end{algorithmic}
\end{algorithm}


  
\begin{algorithm}[t]
\caption{: Analyzer $\mathcal{A}^{\text{Bin}}$ }\label{algo:binary_vector_server}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} $\mathcal{Y}_1,\ldots,\mathcal{Y}_n$, where $\mathcal{Y}_i$ is $s$ messages each is a pair $(z_{ij},y_{ij})$ for $j\in[s]$ and $i\in[n]$. 
\STATE $\hat{\mathbf{b}}\gets \mathbf{0}_{d}$
\FOR{$i\in[n]$}
\FOR{$j\in [s]$}
\STATE $\hat{\mathbf{b}}[z_{ij}]\gets \hat{\mathbf{b}}[z_{ij}]+y_{ij}$.
\ENDFOR
\ENDFOR
\STATE $\hat{\mathbf{b}}\gets \frac{1}{n}\hat{\mathbf{b}}$
\STATE \textbf{Return:} The server returns $\hat{\mathbf{b}}$.
\end{algorithmic}
\end{algorithm}

In the following theorems, we prove the bound on the MSE of the proposed mechanisms in the local DP and shuffle models. The proofs are deferred to Appendix~\ref{app:binary_vector_sum}. For ease of presentation, we provide the order of the achievable MSE and give the $\epsilon_0$-LDP and/or central $\left(\epsilon,\delta\right)$-DP guarantees of our mechanism for both local DP and shuffle models. However, we track the constants in the MSE in the detailed proofs in Appendix~\ref{app:binary_vector}. Furthermore, we present RDP guarantees of our mechanisms for both local DP and shuffle models in the detailed proofs.   
 
\begin{theorem}[Local DP model]~\label{thm:binary_vector_ldp} The output of the local mechanism $\mathcal{R}^{\text{Bin}}_{p,s}$ can be represented using $s\left(\log\left(\lceil d/s\rceil\right)+1\right)$ bits. By choosing $p=\frac{1}{2}\left(1-\sqrt{\frac{\epsilon_0^2/s^2}{\epsilon_0^2/s^2+4}}\right)$, the mechanism $\mathcal{R}_{p,s}^{\text{Bin}}$ satisfies $\epsilon_0$-LDP. Let $\hat{\mathbf{b}}$ be the output of the analyzer $\mathcal{A}^{\text{Bin}}$. The estimator $\hat{\mathbf{b}}$ is an unbiased estimate of $\overline{\mathbf{b}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{b}_i$ with bounded MSE:
\begin{equation}~\label{eqn:mse_binary_vector_ldp}
\begin{aligned}
\mathsf{MSE}^{\text{Bin}}_{\text{ldp}}&=\sup_{\lbrace \mathbf{b}_i\in \lbrace0,1\rbrace^{d}\rbrace}\mathbb{E}\left[\|\hat{\mathbf{b}}-\overline{\mathbf{b}}\|_2^2\right]\\
& = \mathcal{O}\left(\frac{d^2}{n}\max\left\{\frac{1}{s},\frac{s}{\epsilon_0^2}\right\}\right).
\end{aligned}
\end{equation}
\end{theorem}
Observe that Theorem~\ref{thm:binary_vector_ldp} shows that each client needs to send $s=\lceil \epsilon_0 \rceil$ communication bits to achieve MSE $\mathcal{O}\left(\frac{d^2}{n\min\lbrace \epsilon_0,\epsilon_0^2\rbrace}\right)$. Now, we move to the shuffle model, where we assume that there exists $s$ shuffler. The $j$-th shuffler randomly permutes the set of messages $\left\{\left(z_{ij},y_{ij}\right):i\in[n]\right\}$ from the $n$ clients.

\begin{theorem}[Shuffle DP model]~\label{thm:binary_vector_shuffle} The output of the local mechanism $\mathcal{R}^{\text{Bin}}_{p,s}$ can be represented using $s\left(\log\left(\lceil d/s\rceil\right)+1\right)$ bits. For every $n\in\mathbb{N}$, $\epsilon\leq 1$, and $\delta\in (0,1)$, shuffling the outputs of $n$ mechanisms $\mathcal{R}_{p,s}^{\text{Bin}}$ satisfies $\left(\epsilon,\delta\right)$-DP by choosing $p=\frac{1}{2}\left(1-\sqrt{\frac{v^2}{v^2+4}}\right)$, where $v^2=\frac{n\epsilon^2}{4s\log(1/\delta)}$. Let $\hat{\mathbf{b}}$ be the output of the analyzer $\mathcal{A}^{\text{Bin}}$. The estimator $\hat{\mathbf{b}}$ is an unbiased estimate of $\overline{\mathbf{b}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{b}_i$ with bounded MSE:
\begin{equation}~\label{eqn:mse_binary_vector_shuffle}
\begin{aligned}
\mathsf{MSE}^{\text{Bin}}_{\text{shuffle}}&=\sup_{\lbrace \mathbf{b}_i\in \lbrace0,1\rbrace^{d}\rbrace}\mathbb{E}\left[\|\hat{\mathbf{b}}-\overline{\mathbf{b}}\|_2^2\right]\\
& = \mathcal{O}\left(\frac{d^2}{n^2}\max\left\{n\left(\frac{1}{s}-\frac{1}{d}\right),\frac{\log\left(1/\delta\right)}{\epsilon^2}\right\}\right).
\end{aligned}
\end{equation}
\end{theorem}
Observe that Theorem~\ref{thm:binary_vector_shuffle} shows that each client requires to send $s=\mathcal{O}\left(\min\lbrace n\epsilon^2,d\rbrace\right)$ communication bits such that the error in the shuffle model is bounded by $\mathcal{O}\left(\frac{d^2}{n^2\epsilon^2}\right)$ that matches the MSE of central differential privacy mechanisms. For the scalar case when $d=1$, our results in Theorem~\ref{thm:binary_vector_shuffle} matches the optimal MSE as in~\cite{cheu2019distributed}. 


==> L2_norm.tex <==
\section{ Bounded $\ell_2$-norm Vectors}
\label{sec:l_2_norm}

In this section, we consider the bounded $\ell_{2}$-norm, where the $i$th client has a vector $\mathbf{x}_i$ such that $\|\mathbf{x}_i\|_{2}\leq r_{2}$ for $i\in[n]$. We use the random rotation proposed in~\cite{suresh2017distributed} to bound the $\ell_{\infty}$-norm of the vector with radius $r_{\infty}=\mathcal{O}\left(\frac{r_2}{\sqrt{d}}\right)$ and then we apply the bounded $\ell_{\infty}$-norm algorithm in Section~\ref{sec:l_inf_norm}. 





\begin{algorithm}[t]
\caption{: Local Randomizer $\mathcal{R}^{\ell_{2}}_{v,m,s}$ }\label{algo:l_2}
\begin{algorithmic}[1]
\STATE \textbf{Public parameter:} Privacy budget $v$, communication levels $m$, communication coordinates per level $s$, and confidence term $\beta$.
\STATE \textbf{Input:} $\mathbf{x}_i\in \mathbb{B}^{d}_{2}\left(r_{2}\right)$.
\STATE Let $U=\frac{1}{\sqrt{d}}\mathbf{H}D$, where $\mathbf{H}$ denotes a Hadamard matrix and $D$ is a diagonal matrix with i.i.d. uniformly random $\lbrace \pm 1\rbrace$ entries.
\STATE $\mathbf{w}_i\gets W\mathbf{x}_i$
\STATE $r_{\infty}\gets 10r_2\sqrt{\frac{\log\left(dn/\beta\right)}{d}}$
\FOR{$j=1,\ldots,d$}
\STATE $\mathbf{w}_i[j]=\max\left\{-r_{\infty},\min\left\{\mathbf{w}_i(j),r_{\infty}\right\}\right\}$
\ENDFOR
\STATE $\mathcal{Y}_i\gets \mathcal{R}^{\ell_{\infty}}_{v,m,s}(\mathbf{w}_i)$
\STATE \textbf{Return:} The client sends $\mathcal{Y}_i$.
\end{algorithmic}
\end{algorithm}
   
\begin{algorithm}[t]
\caption{: Analyzer $\mathcal{A}^{\ell_{2}}$ }\label{algo:l_2_server}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} $\mathcal{Y}_1,\ldots,\mathcal{Y}_n$, where $\mathcal{Y}_i=\left\{\mathcal{Y}_i^{(1)},\ldots,\mathcal{Y}_i^{(m)}\right\}$ is a set of $m$ sets.
\STATE $\hat{\mathbf{w}}\gets \mathcal{A}^{\ell_{\infty}}\left(\mathcal{Y}_1,\ldots,\mathcal{Y}_n\right)$
\STATE \textbf{Return:} The server returns $\hat{\mathbf{x}}\gets U^{-1}\hat{\mathbf{w}}$.
\end{algorithmic}
\end{algorithm}


\begin{theorem}[Local DP model]~\label{thm:l_2_vector_ldp} The output of the local mechanism $\mathcal{R}^{\ell_{2}}_{v,m,s}$ can be represented using $sm\left(\log\left(\lceil d/s\rceil\right)+1\right)$ bits. By choosing $v=\epsilon_0$, the mechanism $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ satisfies $\epsilon_0$-LDP. Let $\hat{\mathbf{x}}$ be the output of the analyzer $\mathcal{A}^{\ell_{2}}$. With probability at least $1-\beta$, the estimator $\hat{\mathbf{x}}$ is an unbiased estimate of $\overline{\mathbf{x}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{x}_i$ with bounded MSE:
\begin{equation}~\label{eqn:mse_l_2_vector_ldp}
\begin{aligned}
&\mathsf{MSE}^{\ell_{\infty}}_{\text{ldp}}=\sup_{\lbrace \mathbf{x}_i\in\mathbb{B}_{2}^{d}\left(r_{2}\right)\rbrace}\mathbb{E}\left[\|\hat{\mathbf{x}}-\overline{\mathbf{x}}\|_2^2\right]\\
&\quad = \mathcal{O}\left(\frac{r_{2}^{2}d\log\left(dn/\beta\right)}{n}\max\left\{\frac{d}{4^{m}},\frac{d}{s},\frac{ds}{\epsilon_0^2}\right\}\right).
\end{aligned}
\end{equation}
\end{theorem}

\begin{theorem}[Shuffle DP model]~\label{thm:l_2_vector_shuffle} The output of the local mechanism $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ can be represented using $sm\left(\log\left(\lceil d/s\rceil\right)+1\right)$ bits. For every $n\in\mathbb{N}$, $\epsilon\leq 1$, and $\delta\in (0,1)$, the shuffling the outputs of $n$ mechanisms $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ satisfies $\left(\epsilon,\delta\right)$-DP by choosing $v^2=\frac{n\epsilon^2}{s\log(1/\delta)}$. Let $\hat{\mathbf{x}}$ be the output of the analyzer $\mathcal{A}^{\ell_{\infty}}$. With probability at least $1-\beta$ The estimator $\hat{\mathbf{x}}$ is an unbiased estimate of $\overline{\mathbf{x}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{x}_i$ with bounded MSE:
\begin{equation}~\label{eqn:mse_l_2_vector_shuffle}
\begin{aligned}
&\mathsf{MSE}^{\ell_{2}}_{\text{shuffle}}=\sup_{\lbrace \mathbf{x}_i\in\mathbb{B}_{2}^{d}\left(r_{2}\right)\rbrace}\mathbb{E}\left[\|\hat{\mathbf{x}}-\overline{\mathbf{x}}\|_2^2\right]\\
&\quad = \mathcal{O}\left(\frac{r_{2}^{2}\log\left(dn/\beta\right)}{n^2}\max\left\{\frac{n}{4^{m}},n\left(\frac{d}{s}-1\right),\frac{d\log\left(1/\delta\right)}{\epsilon^2}\right\}\right).
\end{aligned}
\end{equation}
\end{theorem}


\section{Lower Bounds}
In this section, we present lower bounds for DME under privacy and communication constraints. The first lower bound for local DP model is proposed in~\cite{chen2020breaking} in Theorem~$2.1$. The second lower bound for the shuffle model is a combination of the lower bound on DME with communication constraints proposed in~\cite{pmlr-v162-chen22c} and the lower bound on DME with central $\left(\epsilon,\delta\right)$-DP constraints proposed in~\cite{bun2014fingerprinting}.


\begin{theorem}[Lower Bound For local DP model~\cite{chen2020breaking}]~\label{thm:L_2_lower_bound_ldp} Let $n,d\in\mathbb{N}$ and $\epsilon_0>0$. For any $\mathbf{x}_1,\ldots,\mathbf{x}_n\in\mathbb{B}_2^{d}(r_2)$, the MSE is bounded below by:
 \begin{equation}
\mathsf{MSE}_{\text{ldp}}^{\ell_2}=\Omega\left(\frac{r_2^2d}{n\min\left\{\epsilon^2_0,\epsilon_0,b \right\}}\right)
\end{equation}
for any unbiased algorithm $\mathcal{M}$ that is $\epsilon_0$-LDP with $b$-bits of communication per client. 
\end{theorem}
 
 
\begin{theorem}[Lower Bound For central DP model~\cite{pmlr-v162-chen22c}+~\cite{bun2014fingerprinting}]~\label{thm:L_2_lower_bound_central} Let $n,d\in\mathbb{N}$, $\epsilon>0$, $r_2\geq1$, and $\delta=o(\frac{1}{n})$. For any $\mathbf{x}_1,\ldots,\mathbf{x}_n\in\mathbb{B}_2^{d}(r_2)$, the MSE is bounded below by:
\begin{equation}
\mathsf{MSE}_{\text{central}}^{\ell_2}=\Omega\left(r_2^2\max\left\{\frac{d}{n^2\epsilon^2},\frac{1}{n4^{b/d}}\right\}\right)
\end{equation}
for any unbiased algorithm $\mathcal{M}$ that is $\left(\epsilon,\delta\right)$-DP with $b>d$-bits of communication per client. Furthermore, when $b<d$ bits per client, the MSE is bounded below by:
 \begin{equation}
\mathsf{MSE}_{\text{central}}^{\ell_2}=\Omega\left(r_2^2d\max\left\{\frac{1}{n^2\epsilon^2},\frac{1}{nb} \right\}\right)
\end{equation}
\end{theorem}


==> Linf_norm.tex <==
\section{Bounded $\ell_{\infty}$-norm vectors}~\label{sec:l_inf_norm}
In this section, we consider the bounded $\ell_{\infty}$-norm, where the $i$th client has a vector $\mathbf{x}_i$ such that $\|\mathbf{x}_i\|_{\infty}\leq r_{\infty}$ for $i\in[n]$. We first scale each vector such that each coordinate becomes bounded in range $\left[0,1\right]$. Then, we decompose each vector into a weighted summation of binary vectors. Finally, we privatize each binary vector using a different privacy budget which leads to an order optimal private mechanism.


Instead of privatizing the vector $\mathbf{x}_i$, each client scales her vector $\mathbf{x}_i$ as follows: $\mathbf{z}_i=\frac{\mathbf{x}_i+r_{\infty}}{2r_{\infty}}$, where the operations are done coordinate-wise. Thus, we have that $\mathbf{z}_{i}[j]\in[0,1]$ for all $j\in[d]$ and $i\in[n]$, where $\mathbf{z}_{i}[j]$ denotes the $j$th coordinate of the vector $\mathbf{z}_{i}$. Observe that the vector $\mathbf{z}_i$ can be decomposed into a weighted summation of binary vectors as follows:
\begin{equation}
\mathbf{z}_i = \sum_{k=1}^{\infty} \mathbf{b}_{i}^{(k)}2^{-k},
\end{equation}  
where $\mathbf{b}_i^{(k)}\in\lbrace 0,1\rbrace^{d}$ for all $k\geq 1$. Each client can recursively construct $\mathbf{b}_i^{(k)}$ as follows. Let $\mathbf{z}_i^{(0)}=\mathbf{0}$ and $\mathbf{z}_i^{(k)}=\sum_{l=1}^{k}\mathbf{b}_i^{(l)}2^{-l}$. Hence, $\mathbf{b}_i^{(k)}=\lfloor 2^{k}\left(\mathbf{z}_i-\mathbf{z}^{(k-1)}_i\right)\rfloor$ for $k\geq 1$.


 To make our mechanism communication efficient, each client approximates the vector $\mathbf{z}_i$ by using the first $m$ binary vectors $\lbrace \mathbf{b}_{i}^{(k)}: 1\leq
 k\leq m\rbrace$. Note that the first $m$ binary vectors give the best approximation to the real vector $\mathbf{z}_i$ with error $\|\mathbf{z}_i-\mathbf{z}^{(m)}_i\|_2^2\leq d/4^{m}$, where $\mathbf{z}^{(m)}_i=\sum_{k=1}^{m}\mathbf{b}_i^{(k)}2^{-k}$. However, this mechanism creates a biased estimate of $\mathbf{z}_i$. Hence, to design an unbiased mechanism, the client approximates the vector $\mathbf{z}_i$ using the first $m-1$ binary vectors $\lbrace \mathbf{b}_{i}^{(k)}:1\leq k\leq m-1\rbrace$ of the binary representation above and the last binary vector ($\mathbf{u}_i$) is reserved for unbiasness as follows:
\begin{equation}
\mathbf{u}_i[j]=\mathsf{Bern}\left(2^{m-1}(\mathbf{z}_{i}[j]-\mathbf{z}_{i}^{(m-1)}[j])\right),
\end{equation}
where $\mathbf{z}^{(m-1)}_i=\sum_{k=1}^{m-1}\mathbf{b}_{i}^{(k)}2^{-k}$ and $\mathsf{Bern}(p)$ denotes Bernoulli random variable with bias $p$. Note that when each client sends the $m$ binary vectors $\lbrace \mathbf{b}_i^{(k)}:1\leq k\leq m-1\rbrace\bigcup \lbrace \mathbf{u}_{i}\rbrace$, the server can generates an unbiased estimate to the mean $\overline{z}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{z}_i$ with error $\mathcal{O}\left(\frac{d}{n4^{m}}\right)$. For completeness, we prove some properties of this quantization scheme in Appendix~\ref{app:quantization}. 

From this binary representation, we can see that the problem of mean of bounded $\ell_{\infty}$-norm vector is converted into a sequence of mean estimation of binary vectors. Hence, each client sends the binary vectors $\lbrace \mathbf{b}_i^{(1)},\ldots, \mathbf{b}_i^{(m-1)}\rbrace$ and $\mathbf{u}_i$ using the binary vector mechanism proposed in~\ref{sec:binary_vector} with different privacy budget  as follows. Observe that the error in estimating the mean of the $k$-th binary vectors $\lbrace b_1^{(k)},\ldots,b_n^{(k)}\rbrace$ contributes in the total MSE by a factor $\mathcal{O}\left(d/4^{k}\right)$. Hence, the goal is to estimate the mean of the $k$-th binary vectors more accurately than estimating the mean of the $j$-th binary vectors for any $j>k$. As a result, we give larger privacy budget (better accuracy) for estimating the mean of the $k$-th binary vectors and smaller privacy budget (less accuracy) for estimating the mean of the $j$-th bit for any $j>k$.

 We present the complete mechanism in Algorithm~\ref{algo:l_inf}, where the input $v$ is to control the total privacy of the mechanism. There are two communication parameters: $m$ controls the approximation level of quantization and $s$ controls the communication bits of sending each binary vector similar to Algorithm~\ref{algo:binary_vector}. In Theorems~\ref{thm:l_inf_vector_ldp} and ~\ref{thm:l_inf_vector_shuffle}, we present how the privacy and communication parameters $v,m,s$ affects the accuracy of the mechanism. The server-side is presented in Algorithm~\ref{algo:l_inf_server}. The server estimate the mean of each binary vectors $\lbrace b_{i}^{(k)}\rbrace$ and decodes the messages to generate an estimate to true mean $\overline{\mathbf{z}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{z}_i$. Then, the server scales the vector $\overline{\mathbf{z}}$ to generate an unbiased estimate of the mean $\overline{\mathbf{x}}$.


\begin{algorithm}[t]
\caption{: Local Randomizer $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ }\label{algo:l_inf}
\begin{algorithmic}[1]
\STATE \textbf{Public parameter:} Privacy budget $v$, communication levels $m$, and communication coordinates per level $s$.
\STATE \textbf{Input:} $\mathbf{x}_i\in \mathbb{B}^{d}_{\infty}\left(r_{\infty}\right)$.
\STATE $\mathbf{z}_i \gets \left(\mathbf{x}_i+r_{\infty}\right)/2r_{\infty}$
\STATE $\mathbf{z}^{(0)}_i\gets 0$
\FOR{$k=1,\ldots,m-1$}
\STATE $\mathbf{b}_i^{(k)}\gets \lfloor 2^{k}(\mathbf{z}_i-\mathbf{z}^{(k-1)}_i)\rfloor$
\STATE $v_k \gets \frac{4^{\frac{-k}{3}}}{\left(\sum_{l=1}^{m-1}4^{\frac{-l}{3}}+4^{\frac{-m+1}{3}}\right)} v$
\STATE $p_k\gets \frac{1}{2}\left(1-\sqrt{\frac{v_k^2/s^2}{v_k^2/s^2+4}}\right)$
\STATE $\mathcal{Y}_i^{(k)}\gets \mathcal{R}^{\text{Bin}}_{p_k,s}(\mathbf{b}_i^{(k)})$
\STATE $\mathbf{z}^{(k)}_i\gets \mathbf{z}^{(k-1)}_i+\mathbf{b}_i^{(k)}2^{-k}$
\ENDFOR
\STATE Sample $\mathbf{u}_i\gets \mathsf{Bern}\left(2^{m-1}\left(\mathbf{z}_i-\mathbf{z}^{(m-1)}_i\right)\right)$
\STATE $v_m \gets \frac{4^{\frac{-m+1}{3}}}{\left(\sum_{l=1}^{m-1}4^{\frac{-l}{3}}+4^{\frac{-m+1}{3}}\right)}v$
\STATE $p_m\gets \frac{1}{2}\left(1-\sqrt{\frac{v_m^2/s^2}{v_m^2/s^2+4}}\right)$
\STATE $\mathcal{Y}_i^{(m)}\gets \mathcal{R}^{\text{Bin}}_{p_m,s}(\mathbf{u}_i)$
\STATE \textbf{Return:} The client sends $\mathcal{Y}_i\gets\left\{\mathcal{Y}_i^{(1)},\ldots,\mathcal{Y}_i^{(m)}\right\}$.
\end{algorithmic}
\end{algorithm}
   
\begin{algorithm}[t]
\caption{: Analyzer $\mathcal{A}^{\ell_{\infty}}$ }\label{algo:l_inf_server}
\begin{algorithmic}[1]
\STATE \textbf{Inputs:} $\mathcal{Y}_1,\ldots,\mathcal{Y}_n$, where $\mathcal{Y}_i=\left\{\mathcal{Y}_i^{(1)},\ldots,\mathcal{Y}_i^{(m)}\right\}$ is a set of $m$ sets.
\FOR {$k=1,\ldots,m-1$}
\STATE $\hat{\mathbf{b}}^{(k)}\gets\mathcal{A}^{\text{Bin}}\left(\mathcal{Y}_1^{(k)},\ldots,\mathcal{Y}_n^{(k)}\right)$
\ENDFOR
\STATE $\hat{\mathbf{u}}\gets\mathcal{A}^{\text{Bin}}\left(\mathcal{Y}_1^{(m)},\ldots,\mathcal{Y}_n^{(m)}\right)$
\STATE $\hat{\mathbf{z}}\gets \sum_{k=1}^{m-1}\hat{\mathbf{b}}^{(k)}2^{-k}+\hat{\mathbf{u}}2^{-m+1}$ 
\STATE \textbf{Return:} The server returns $\hat{\mathbf{x}}\gets 2r_{\infty}\hat{\mathbf{z}}-r_{\infty}$.
\end{algorithmic}
\end{algorithm}

 We prove the bound on the MSE of the proposed mechanisms in the local DP and shuffle models in the following theorems, where we defer the proofs to Appendix~\ref{app:l_inf_vector}. For ease of presentation, we provide the order of the achievable MSE and give the $\epsilon_0$-LDP and/or central $\left(\epsilon,\delta\right)$-DP guarantees of our mechanism for both local DP and shuffle models. Similar to the binary vectors, we track the constants in the MSE in the detailed proofs in Appendix~\ref{app:l_inf_vector} (see \eqref{eq:ExpConst-MSE-linf-LDP}, \eqref{eq:ExpConst-MSE-lind-MMS}. Furthermore, we present RDP guarantees of our mechanisms for both local DP and shuffle models in the detailed proofs.   
 
\begin{theorem}[Local DP model]~\label{thm:l_inf_vector_ldp} The output of the local mechanism $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ can be represented using $ms\left(\log\left(\lceil d/s\rceil\right)+1\right)$ bits. By choosing $v=\epsilon_0$, the mechanism $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ satisfies $\epsilon_0$-LDP. Let $\hat{\mathbf{x}}$ be the output of the analyzer $\mathcal{A}^{\ell_{\infty}}$. The estimator $\hat{\mathbf{x}}$ is an unbiased estimate of $\overline{\mathbf{x}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{x}_i$ with bounded MSE:
\begin{equation}~\label{eqn:mse_l_inf_vector_ldp}
\begin{aligned}
\mathsf{MSE}^{\ell_{\infty}}_{\text{ldp}}&=\sup_{\lbrace \mathbf{x}_i\in\mathbb{B}_{\infty}^{d}\left(r_{\infty}\right)\rbrace}\mathbb{E}\left[\|\hat{\mathbf{x}}-\overline{\mathbf{x}}\|_2^2\right] \\
&= \mathcal{O}\left(\frac{r_{\infty}^{2}d^2}{n}\max\left\{\frac{1}{d4^{m}},\frac{1}{s},\frac{s}{\epsilon_0^2}\right\}\right).
\end{aligned}
\end{equation}
\end{theorem}
Observe that Theorem~\ref{thm:l_inf_vector_ldp} shows that each client needs to set $m=1$ and $s=\lceil \epsilon_0 \rceil$ communication bits to achieve MSE $\mathcal{O}\left(\frac{d^2}{n\min\lbrace \epsilon_0,\epsilon_0^2\rbrace}\right)$ when $\epsilon_0\leq \sqrt{d}$. Now, we move to the shuffle model, where there is a secure shuffler that randomly permutes the private messages of the clients before passing them to the server. 

\begin{theorem}[Shuffle DP model]~\label{thm:l_inf_vector_shuffle} The output of the local mechanism $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ can be represented using $ms\left(\log\left(\lceil d/s\rceil\right)+1\right)$ bits. For every $n\in\mathbb{N}$, $\epsilon\leq 1$, and $\delta\in (0,1)$, the shuffling the outputs of $n$ mechanisms $\mathcal{R}^{\ell_{\infty}}_{v,m,s}$ satisfies $\left(\epsilon,\delta\right)$-DP by choosing $v^2=\frac{sn\epsilon^2}{4\log(1/\delta)}$. Let $\hat{\mathbf{x}}$ be the output of the analyzer $\mathcal{A}^{\ell_{\infty}}$. The estimator $\hat{\mathbf{x}}$ is an unbiased estimate of $\overline{\mathbf{x}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{x}_i$ with bounded MSE:
\begin{equation}~\label{eqn:mse_l_inf_vector_shuffle}
\begin{aligned}
&\mathsf{MSE}^{\ell_{\infty}}_{\text{shuffle}}=\sup_{\lbrace \mathbf{x}_i\in\mathbb{B}_{\infty}^{d}\left(r_{\infty}\right)\rbrace}\mathbb{E}\left[\|\hat{\mathbf{x}}-\overline{\mathbf{x}}\|_2^2\right]\\
&\ = \mathcal{O}\left(\frac{r_{\infty}^{2}d^2}{n^2}\max\left\{\frac{n}{d4^{m}},n\left(\frac{1}{s}-\frac{1}{d}\right),\frac{\log\left(1/\delta\right)}{\epsilon^2}\right\}\right).
\end{aligned}
\end{equation}
\end{theorem}
Observe that Theorem~\ref{thm:l_inf_vector_shuffle} shows that each client requires to set $m=\lceil \log\left(n\epsilon^2/d\right)\rceil$ and $s=\mathcal{O}\left(\min\lbrace n\epsilon^2,d\rbrace\right)$ such that the error in the shuffle model is bounded by $\mathcal{O}\left(\frac{d^2}{n^2\epsilon^2}\right)$ that matches the MSE of central differential privacy mechanisms.

 
 


==> Problem_formulation.tex <==
\section{Problem Formulation}
In this section, we present the problem formulation.
\subsection{Federated Learning}
We study federated learning (FL) framework, where a set of $n$ clients are connected to an untrusted server to solve the empirical risk minimization (ERM) problem:
\begin{equation}
\min_{\mathbf{w}} F\left(\mathbf{w}\right)=\frac{1}{n}\sum_{i=1}^{n}F_i\left(\mathbf{w}\right),
\end{equation}
where $\mathbf{w}\in\mathbb{R}^{d}$ denotes the optimization model, and $F_i\left(\mathbf{w}\right)=\mathbb{E}_{d_i\sim\mathcal{D}_i}\left[F_i\left(\mathbf{w},d_i\right)\right]$ denotes the loss function of the $i$-th client. Perhaps \textsf{FedAvg}~\cite{} is the most common algorithm in FL. At the $t$th round, the server send the current model $\mathbf{w}_t$ to the sampled clients $\mathcal{S}_t$. Each client $i\in\mathcal{S}_t$ runs local updates and returns the local gradients $\nabla F_i\left(\mathbf{w}_t\right)$ to the server to update the model $w_{t+1}=w_{t}-\eta \frac{1}{m}\sum_{i\in\mathcal{S}_t}\nabla F_i\left(\mathbf{w}_t\right)$, where $\eta$ is the learning rate and $\mathcal{S}_t$ is the set of sampled client at round $t$ of size $|\mathcal{S}_t|=m$. Hence, a communication-efficient and private FL algorithm can be obtained from designing an optimal mechanism of distributed mean estimation (DME). 

\subsection{Distributed Mean Estimation (DME)}
We study the distributed mean estimation problem under privacy and communication constraints. Suppose we have a set of $n$ clients. Each client has has a $d$ dimensional vector $\mathbf{x}_i\in\mathcal{X}$ for $i\in[n]$, where $\mathcal{X}\subset\mathbb{R}^{d}$ denotes a bounded subset of all possible inputs. For example, $\mathcal{X}\triangleq \mathbb{B}^{d}_2(r_2)$ denotes the $d$ dimensional ball with radius $r_2$, i.e., each vector $\mathbf{x}_i$ satisfies $\|\mathbf{x}_i\|_2\leq r_2$ for $i\in[n]$. Furthermore, each client has a communication budget of $b$-bits. The clients are connected to an (untrusted) server that wants to estimate the mean $\overline{\mathbf{x}}=\frac{1}{n}\sum_{i=1}^{n}\mathbf{x}_i$.

In this paper, we consider two different privacy models. Both models are distributed. In addition, we assume that the server is untrusted, and hence, each client privatize her own data before sending it. 
\subsection{Local DP Model} In the local DP model, our goal is to design two mechanisms: 1) A client-side mechanism $\mathcal{R}:\mathcal{X}\to\mathcal{Y}$. 2) Server aggregator $\mathcal{A}:\mathcal{Y}^{n}\to \mathbb{R}^{d}$. The local mechanism $\mathcal{R}$ takes an input $\mathbf{x}_i\in\mathcal{X}$ and generates a randomized output $\mathbf{y}_i\in\mathcal{Y}$, where the output $\mathbf{y}_i$ can be a set of multiple messages. The local mechanism $\mathcal{R}$ satisfies privacy and communication constraints as follows. The output $\mathbf{y}_i=\mathcal{R}\left(\mathbf{x}_i\right)$ can be represented using only $b$-bits. Furthermore, the mechanism $\mathcal{R}$ satisfies $\epsilon_0$-LDP (see Definition~\ref{defn:LDPdef}). Each client sends the output $\mathbf{y}_i$ directly to the server. The server applies the aggregator $\mathcal{A}$ to estimate the mean $\hat{\mathbf{x}}=\mathcal{A}\left(\mathbf{y}_1,\ldots,\mathbf{y}_n \right)$ such that the estimated mean $\hat{\mathbf{x}}$ is an unbiased estimate of the true mean $\overline{\mathbf{x}}$.

\subsection{Shuffle Model}
The shuffle model is similar to the local DP model except the existence of a secure shuffler between the clients and the server, where shuffling can amplify the privacy of the algorithm. Precisely, the shuffle model consists of three parameters $\left(\mathcal{R},\mathcal{S},\mathcal{A}\right)$: \textit{1) Encode:} a local mechanism $\mathcal{R}:\mathcal{X}\to\mathcal{Y}$ similar to the local DP model. Each client sends the output $\mathbf{y}_i$ to the secure shuffler. \textit{2) Shuffle:} a secure shuffler $\mathcal{S}:\mathcal{Y}^{n}\to \mathcal{Y}^{n}$ receives $n$ outputs after applying the local mechanism $\mathcal{R}$ on each input $\mathbf{x}_1,\ldots,\mathbf{x}_n$ and generates a random permutation of the received messages. \textit{3) Analyze:} the server receives the shuffled messages and applies the aggregator $\mathcal{A}:\mathcal{Y}^{n}\to \mathbb{R}^{d}$ to estimate the mean $\hat{\mathbf{x}}=\mathcal{A}\left(\mathbf{y}_{\pi(1)},\ldots,\mathbf{y}_{\pi(n)}\right)$.
We say that the shuffled model is $\left(\epsilon,\delta\right)$-DP if the view of the output of the shuffler $\left(\mathbf{y}_1,\ldots,\mathbf{y}_n\right)$ satisfies $\left(\epsilon,\delta\right)$-DP. Observe that the local mechanism $\mathcal{R}$ doesn't need to satisfy $\epsilon_0$-LDP, however, it is required to satisfy the communication constraints. Furthermore, we need to design $\mathcal{R}$ such that the output of the shuffler is $\left(\epsilon,\delta\right)$-DP

In the two privacy models, the performance of the estimator $\hat{\mathbf{x}}$ is measured by the expected loss:
\begin{equation}~\label{eqn:loss}
\mathsf{MSE}= \sup_{\lbrace\mathbf{x}_i\in\mathcal{X}\rbrace}\mathbb{E}\left[\|\hat{\mathbf{x}}-\overline{\mathbf{x}}\|_2^2\right],
\end{equation}
where the expectation is taken over the randomness of the private mechanisms. Hence, our goal is to design communication-efficient and private schemes to generate an unbiased estimate of the true mean $\overline{x}$ while minimizing the expected loss~\eqref{eqn:loss}. We propose a local mechanism $\mathcal{R}$ and a server aggregator $\mathcal{A}$, where we show that these mechanisms achieve optimal privacy and communication efficiency in both privacy models (local DP and shuffle models).

 We start by studying the problem of mean estimation of binary vectors, where $\mathcal{X}\triangleq \lbrace0,1\rbrace^d$. Next, we study the bounded $\ell_{\infty}$-norm case such that $\mathcal{X}\triangleq \mathbb{B}^{d}_{\infty}(r_{\infty})$, i.e., $\|\mathbf{x}_i\|_{\infty}\leq r_{\infty}$ for all $i\in[n]$. For bounded $\ell_2$-norm vectors when $\mathcal{X}\triangleq \mathbb{B}^{d}_2(r_2)$, we use the random rotation technique proposed in~\cite{suresh2017distributed} to bound the $\ell_{\infty}$-norm of each coordinate with radius $r_{\infty}=\mathcal{O}\left(\frac{r_2}{\sqrt{d}}\right)$ and then we apply the $\ell_{\infty}$-norm algorithm. 


==> RelatedWork.tex <==
%\noindent\textbf{Trade-offs in locally private DME:}
There has been a significant amount of recent interest in private mean
estimation for local DP guarantees(\emph{e.g.,}
~\cite{chen2020breaking,girgis2021shuffled,PrivUnit-based,Kamalika}),
where order optimal solutions have been proposed. Our local DP methods
also achieve this trade-off using a different mechanism, which also
can be easily adapted to the MMS model. As mentioned the local privacy
suffers from worse privacy-performance tradeoffs \cite{GiveRefs-from
AISTATS} as compared to methods that use privacy amplification such as
SecAgg or MMS. Our results on private DME in the MMS model closely
relate to works in \cite{MMS-refs}. The private \emph{scalar} DME was
studied in \cite{Scalar-MMS}, where order optimal strategies (for some
regimes) were established. The private vector DME has received less
attention, with the exception of \cite{Cheu-VecSum}. Our private
vector DME results in Theorem *** improve the
privacy-communication-performance order-wise over it (see Remark
***). Also as mentioned earlier our scheme is order-wise optimal for all
regimes. Though we study a different privacy model through shuffling (MMS), the SecAgg framework is an alternate methodlogy to overcome the deficiencies of pure local privacy. This was studied in \cite{GoogleICML22}, where an order-optimal private DME for SecAgg was established. Using the alternative MMS framework we achieve order-wise same behavior. but for all regimes, and our scheme can potentially be more communication efficient than the local scheme \cite{DDG} used in \cite{GoogleICML22}. There has been a lot of work on private optimization both in the local model \cite{PrivOptLocal} and in the shuffled models \cite{AISTATS21,NeurIPS21,CheuICLR22}. Our result on private optimization builds directly on the private DME results to give better overall privacy-communication-performance operating points. We give a more detailed accounting of all the related literature in the Appendix \ref{app:RelWork}.


%Ayfer, Vitaly, AISTATS21, DDG, other works

%\noindent\textbf{Multi-message shuffled models:}
%Scalar case, vector case

%\noindent\textbf{Secure Aggregation:}

%\noindent\textbf{Private optimization:}
%AISTATS21, NeurIPS21, CCS21, Erlingson-Vitaly etc.


==> app_Priv-defs.tex <==
\section{Privacy: definitions, composition and conversions}\label{app_sec:Priv-defs}
In this section, we define different privacy notions that we will use in this paper: local differential privacy (LDP), central different privacy (DP), and Renyi differential privacy (RDP). We also give standard results on privacy composition as well as conversion between privacy notions.

\begin{definition}[Local Differential Privacy - LDP~\citep{kasiviswanathan2011can}]~\label{defn:LDPdef}
For $\epsilon_0\geq0$, a randomized mechanism $\calR:\calX\to\calY$ is said to be $\eps_0$-local differentially private (in short, $\eps_{0}$-LDP), if for every pair of inputs $d,d'\in\calX$, we have 
\begin{equation}~\label{app:ldp-def}
\Pr[\calR(d)\in \calS] \leq e^{\eps_0}\Pr[\calR(d')\in \calS], \qquad \forall \calS\subset\calY.
\end{equation}
\end{definition}
Let $\calD=\lbrace d_1,\ldots,d_n\rbrace$ denote a dataset comprising $n$ points from $\mathcal{X}$. We say that two datasets $\calD=\lbrace d_1,\ldots,d_n\rbrace$ and $\calD^{\prime}=\lbrace d_1^{\prime},\ldots,d_n^{\prime}\rbrace$ are neighboring (and denoted by $\calD\sim\calD'$) if they differ in one data point, i.e., there exists an $i\in[n]$ such that $d_i\neq d'_i$ and for every $j\in[n],j\neq i$, we have $d_j=d'_j$.
\begin{definition}[Central Differential Privacy - DP \citep{Calibrating_DP06,dwork2014algorithmic}]\label{defn:central-DP}
For $\epsilon,\delta\geq0$, a randomized mechanism $\calM:\calX^n\to\calY$ is said to be $(\epsilon,\delta)$-differentially private (in short, $(\epsilon,\delta)$-DP), if for all neighboring datasets $\calD\sim\calD^{\prime}\in\calX^{n}$ and every subset $\calS\subseteq \calY$, we have
\begin{equation}~\label{dp_def}
\Pr\left[\calM(\calD)\in\calS\right]\leq e^{\eps_0}\Pr\left[\calM(\calD^{\prime})\in\calS\right]+\delta.
\end{equation}
\end{definition}

\begin{definition}[$(\alpha,\epsilon(\alpha))$-RDP (Renyi Differential Privacy)~\cite{mironov2017renyi}]\label{defn:RDP}
A randomized mechanism $\calM:\calX^n\to\calY$ is said to have $\epsilon(\alpha)$-Renyi differential privacy of order $\alpha\in(1,\infty)$ (in short, $(\alpha,\epsilon(\alpha))$-RDP), if for any neighboring datasets $\calD\sim\calD'\in\calX^n$, we have that $D_{\alpha}(\calM(\calD)||\calM(\calD'))\leq \epsilon(\alpha)$, where $D_{\alpha}(P||Q)$ denotes the Renyi divergence between two distributions $P$ and $Q$ defined by: 
\begin{equation}
D_{\alpha}(P||Q)=\frac{1}{\alpha-1}\log\left(\mathbb{E}_{\theta\sim Q}\left[\left(\frac{P(\theta)}{Q(\theta)}\right)^{\alpha}\right]\right),
\end{equation}
\end{definition}
%
The RDP provides a tight privacy accounting of adaptively composed
mechanisms.  The following result states that if we adaptively compose
two RDP mechanisms with the same order, their privacy parameters add
up in the resulting mechanism.

\begin{lemma}[Adaptive composition of RDP~{\cite{mironov2017renyi}}]\label{lemm:compostion_rdp} 
For any $\alpha>1$, let $\calM_1:\calX\to \calY_1$ be a $(\alpha,\epsilon_1(\alpha))$-RDP mechanism and $\calM_2:\calY_1\times \calX\to \calY$ be a $(\alpha,\epsilon_2(\alpha))$-RDP mechanism. Then, the mechanism defined by $(\calM_1,\calM_2)$ satisfies $(\alpha,\epsilon_1(\alpha)+\epsilon_2(\alpha))$-RDP. 
\end{lemma}

We use the following result for converting the RDP guarantees of a
mechanism to its DP guarantees.
\begin{lemma}[From RDP to DP~\cite{canonne2020discrete,Borja_HypTest-RDP20}]\label{lem:RDP_DP} 
Suppose for any $\alpha>1$, a mechanism $\calM$ is $\left(\alpha,\epsilon\left(\alpha\right)\right)$-RDP. For any $\delta>0$, the mechanism $\calM$ is $\left(\epsilon_{\delta},\delta\right)$-DP, where $\epsilon(\delta)$ is given by: 
\begin{equation*}
\begin{aligned}
 & \epsilon_{\delta} = \min_{\alpha} \epsilon\left(\alpha\right)+\frac{\log\left(1/\delta\right)}{\alpha-1}+\log\left(1-1/\alpha\right)\\
\end{aligned}
\end{equation*}
\end{lemma}


==> app_RelWork.tex <==
\section{Related work} \label{app:RelWork}
We give the most relevant work related to the paper and review some of their connections to our work.

\paragraph{Private DME:} In \cite{chen2020breaking,girgis2021shuffled-aistats} the privacy-communication-performance tradeoff were studied both through schemes as well as lower bounds for the local DP model. \cite{chen2020breaking} established the order optimal private DME under local DP model for bounded $\ell_2$-norm vectors. \cite{girgis2021shuffled-aistats} established order optimal private DME for local DP for bounded $\ell_{\infty}$-norm and separately for bounded $\ell_2$-norm vectors. It also extended its use in the single-shuffled model and private optimization framework (see below). In~\cite{guo2022interpolated,chaudhuri2022privacy}, a family of communication-efficient mechanisms is proposed under LDP constraints in federated learning.

In the multi-message shuffled (MMS) model, the private \emph{scalar} DME was
studied in \cite{Balle-MMS-CCS20,Ghazi-Eurocrypt21}, where order optimal strategies (for some
regimes) were established. The private vector DME has received less
attention, with the exception of \cite{Cheu-ICLR22}. Our private
vector DME result in Theorem \ref{thm:l_2_vector_shuffle} improves the
privacy-communication-performance order-wise over it.

In \cite{DDG-ICML21,pmlr-v162-chen22c}, the privacy-communication-performance trade-off in the SecAgg privacy model was studied. In particular, using ideas from compressive sensing, \cite{pmlr-v162-chen22c} established an order-optimal private DME for SecAgg.

\paragraph{Private optimization in the shuffled model:}
There has been a lot of work on private optimization in the local
model, see \cite{agarwal2018cpsgd,girgis2021shuffled-aistats} and references
therein. We will focus on private optimization in the shuffled model,
where there is relatively less work.  Recently~\cite{ESA}
and~\cite{girgis2021shuffled-aistats,girgis2021shuffled-jsait} have
proposed DP-SGD algorithms for federated learning, in the shuffled
model, where at each iteration, each client applies an LDP mechanism
on the gradients. \cite{girgis2021renyi_neurips} studied a private
optimization framework using RDP and additionally evaluated
subsampling (of clients) in the shuffled model. The approach in
~\cite{ESA} was to send full-prevision gradients without compression,
but ~\cite{girgis2021shuffled-aistats,girgis2021renyi_neurips} did use
compression for the gradients. These methods achived certain optimal
privacy-communication-performance operating points, but not in all
regimes. The use of RDP for establishing compositional bounds for
interactive optimization was studied in
\cite{girgis2021renyi-CCS,feldman2022stronger}, which is used in
establishing the privacy bounds for iterative stochastic
optimization. All these were for the single-shuffle model. For the
multi-message shuffled (MMS) model, private optimization was studied
in \cite{Cheu-ICLR22}, which at its core used a private vector DME
with MMS. As explained earlier, our private vector DME is orderwise
better than this scheme, and if we plug our scheme into the standard
convergence analyses for optimization, we obtain better results as
also given in Appendix \ref{app:OptRes}.

